A Large-scale Study on Unsupervised Outlier Model Selection: Do Internal Strategies Suffice?

Given an unsupervised outlier detection task, how should one select a detection algorithm as well as its hyperparameters (jointly called a model)? Unsupervised model selection is notoriously difficult, in the absence of hold-out validation data with ground-truth labels. Therefore, the problem is vastly understudied. In this work, we study the feasibility of employing internal model evaluation strategies for selecting a model for outlier detection. These so-called internal strategies solely rely on the input data (without labels) and the output (outlier scores) of the candidate models. We setup (and open-source) a large testbed with 39 detection tasks and 297 candidate models comprised of 8 detectors and various hyperparameter configurations. We evaluate 7 different strategies on their ability to discriminate between models w.r.t. detection performance, without using any labels. Our study reveals room for progress -- we find that none would be practically useful, as they select models only comparable to a state-of-the-art detector (with random configuration).

==> TABLE/pval-oneshot.tex <==
\begin{table}[H]
%	\vspace{-0.2in}
	\footnotesize
\centering
	\caption{%$p$-values by one-sided paired Wilcoxon signed rank test, mean, standard deviation, and smallest $q$-th model with no significant difference, comparing 
		Variants of one-shot consensus methods %and variants of similarity measures as compared to 
		vs.  baselines.
		%Symbols $\blacktriangle$ and $\triangledown$ % \textBF
		%Values in \textbf{bold} (\underline{underlined}) highlight the cases where method on row is significantly \textbf{better} (\underline{worse}) than method on column at $p$$<$$0.05$.
		 %\reminder{column row names, remove 0 before .} 
	 } % title of Table
%	\vspace{0.1in}	
	   \scalebox{0.9}{
	   	%\hspace{-.2in}
	   		\begin{tabular}{lcc|cc|r}
	   			% 
	   			\toprule
	   				 & \rnd & \ifr & mean AP & std AP & \qap \\
	   			\midrule	 
				\udr-${\rho}$ & \textBF{0.0123} & 0.9052 & {0.383}& {0.283} & {104} \\
				\udr-$\tau$ & \textBF{0.0188} & \underline{0.9516}	& 0.379	& 0.282	& 109\\
				\udr-$NDCG$ & \underline{0.9966} & \underline{1.0000}	& 0.253	& 0.259	& 197\\
				\midrule
				\mc-${\rho}$& \textBF{0.0003} & 0.2173	& 0.395	& 0.289	& 89\\
				\mc-${\tau}$& \textBF{0.0018} & 0.0624	& {0.396}	& {0.297}	& {81} \\
				\mc-${NDCG}$& \underline{0.9995} & \underline{1.0000}	& 0.199	& 0.213
					& 238\\
				\midrule
				\mcs-${\rho}$& \textBF{0.0019} & 0.1935 	& {0.395}	& {0.300}	& {86}\\
				\mcs-${\tau}$& \textBF{0.0018} & 0.8178 	& 0.388	& 0.295	& 100\\
				\mcs-${NDCG}$&  \underline{0.9997} & \underline{1.0000}	& 0.193	& 0.210 & 245
					\\
				\bottomrule
	   		\end{tabular}
}
	\label{table:pvaloneshot} % is used to refer this table in the text
%	\vspace{-0.3in}
\end{table}






==> TABLE/pvalues-cluster.tex <==
\begin{table}[!t]
\centering
	\caption{ Title } % title of Table
	   \scalebox{1}{
	\begin{tabular}{lllll} % centered columns (12 columns)
	    \toprule
		\textbf{Method} &  \textbf{q} & \textbf{Mean AP} & \textbf{Std AP} \\
		
	\end{tabular}}
	\label{table:q} % is used to refer this table in the text
\end{table}






==> TABLE/pvalues-ireos.tex <==
\begin{table}[!t]
\centering
	\caption{ Title } % title of Table
	   \scalebox{1}{
	\begin{tabular}{lllll} % centered columns (12 columns)
	    \toprule
		\textbf{Method} &  \textbf{q} & \textbf{Mean AP} & \textbf{Std AP} \\
		
	\end{tabular}}
	\label{table:q} % is used to refer this table in the text
\end{table}






==> TABLE/smallestq-all_copy.tex <==
\begin{table}[!t]
\centering
	\caption{Summary of results: smallest $q$-th best model with no significant difference, $p$-values by one-sided paired Wilcoxon signed rank test comparing all methods to the baselines, and mean/standard deviation AP across datasets. 
	} % title of Table
	   \scalebox{0.75}{
	\begin{tabular}{c|lrcc|rr} % centered columns (4 columns)
	    \toprule
		& \textbf{Method} & \qap & mean AP & std AP &  \qroc & \qprn \\
		\midrule
		\multirow{13}{*}{\rotatebox[origin=c]{90}{\parbox[c]{5cm}{\centering Stand-alone}}}
		& \xb,\rs,\ch   &	127 & 0.354 & 0.298 & 138 & 91\\
		& \std   	& 231 & 0.223 & 0.228 & 250 & 224\\
		&\h 	 	& 131& 0.299& 0.250 & 177 & 122\\
	%	&\ch 	 	& 127 & 0.354 & 0.298	 & & \\
		 	&\s 	 	& 163 & 0.289& 0.268
		 & 213 & 129\\
		&\iind 	 	& 139& 0.299& 0.248
		 &178 & 124\\
		 &\db 	 	& 123& 0.343& 0.296 & 166& 115\\
		% &\xb 	 	& 127& 0.354& 0.298	 & & \\
		 &\sd 	 	& 156& 0.295& 0.254
		 & 187& 158\\
		&\dunn	 	& 120& 0.350& 0.296
		 & 143& 108\\
 		\cline{2-7}
 		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 		&\emmes & 115 &0.322 & 0.265& 142& 119\\
 		&\mv & 120 &  0.311 & 0.262 & 147& 133\\
 		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 		\cline{2-7}
 		&\ireos	 & 175 & 0.261 & 0.242
 		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 		 &  & \\
 		\hline
 		\multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Consensus}}}
 		&\udr-${\rho}$& 104& 0.383 & 0.283 & 82 & 115\\
 		&\mc-${\tau}$& 81& 0.396 & 0.297 & 91 & 103\\
 		&\mcs-${\rho}$& 86& 0.395 & 0.300 & 99 & 104\\
 			\cline{2-7}
 			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 		&\hits&95 & 0.397& 0.299
 		 & 97 & 99\\
 		&\ens& 81 &0.371& 0.282
 		 & 86 & 92\\
 		 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 		 	\hline
 		 	\multirow{2}{*}{\rotatebox[origin=c]{90}{\parbox[c]{0.6cm}{\centering Agg.}}}	
 		 	&\hitsc& 94& 0.401& 0.286 &77 & 89\\
 		 &\ensc& 79 & 0.373 & 0.282	 
 		 & 87 & 89\\
 		 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 		 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 			\hline	\hline
 			\multirow{2}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering Base.}}}	
 		&\rand 	& 144& 0.342 & 0.234 &  183& 153\\
 		&\ifor 	& 84 & 0.399 & 0.300 &   102&  91\\
 	%	\midrule
 	%		&\top 	& 1 & &  &   1 &  1\\
 		\bottomrule
	\end{tabular}}
	\label{table:q} % is used to refer this table in the text
\end{table}





